CausalDS: Benchmarking Causal Reasoning in Data-Science Agents

Large language models (LLMs) increasingly act as data-science agents, combining abstract reasoning with advanced tool use. Yet the relevant benchmark landscape largely divides into symbolic causal reasoning benchmarks without realistic data analysis or data analysis benchmarks without causal data-generating structure or a range of causal data science tasks. Existing causal evaluation datasets are often restricted to curated examples from existing sources, with diversity coming from limited templatized variations rather than from systematic generation of novel synthetic causal structures. We introduce CausalDS, a benchmark for evaluating causal reasoning in agentic data-science workflows. Each benchmark instance is a scene consisting of a sampled structural causal model (SCM) with generated observational data and an accompanying synthetic natural-language story grounded in a real domain. We ground the composition of the benchmark components in empirical distributions obtained from real-world datasets, thus retaining empirical structure while reducing the memorization risk through completely synthetic generation. From each scene, we then derive tasks spanning all three of Pearl's rungs. Most tasks include a data science coding component, where the model typically needs to use several tools to arrive at the final answer due to imperfect observations. Abstention is tested directly: for targets the graph does not identify, the graded answer is to abstain. The benchmark thus jointly evaluates symbolic causal reasoning, data science, uncertainty quantification, abstention, and tool use/coding. Because the generator is fully synthetic, the exam is not a fixed dataset: composition, difficulty, and size are parameters, and fresh exams can be drawn at will.

==> figs/scene_example_content.tex <==
% Editable manuscript Figure 2 content.
% Update the story, data rows, question, variable key, and DAG here.
\newcommand{\SceneTitle}{Irrigation and soil erosion}
\newcommand{\SceneMetadata}{R2 bias diagnostic\enspace\textperiodcentered\enspace forbidden-controls output variant\enspace\textperiodcentered\enspace \texttt{iv} motif\enspace\textperiodcentered\enspace hard observation variant}

\newcommand{\SceneStory}{%
Farmers in a semi-arid region receive an Irrigation Activation Subsidy (dollars per hectare) that economically incentivizes whether an Irrigation Event is Executed on their cropland. This decision also depends on the Subsurface Soil Permeability---an unobserved property (cm/hour) that remains latent to agricultural economists but governs how water infiltrates the soil: a sufficient subsidy together with permeable subsoil switches the binary Irrigation Event Executed to 1, while an insufficient subsidy or impermeable subsoil yields 0. The Field Soil Erosion Rate (tons per hectare per year) is the outcome: executing an irrigation event mechanically disturbs and displaces topsoil and raises erosion, while the Subsurface Soil Permeability exerts its own direct effect---higher permeability minimizes surface runoff and soil loss, lower permeability intensifies it. The observed erosion rate thus reflects both the irrigation intervention and the unobserved soil hydraulics.%
}

\newcommand{\SceneDataDescription}{%
$Z_1,\dots,Z_3$ are noisy measurements of the conceptual variable Irrigation Activation Subsidy; $X_1,\dots,X_3$ are noisy measurements of the conceptual variable Irrigation Event Executed.%
}

\newcommand{\SceneDataRows}{%
  0.4  &  2.2 &  0.2 &  0.5 & -2.2 & 0 & 2.4 \\
 -0.8  & -2.4 & -0.9 & -0.3 & -1.5 & 1 & 1.6 \\
  4.0  &  2.9 & -0.3 &  0.7 & -0.2 & 0 & 3.0 \\
}

\newcommand{\SceneQuestion}{%
For estimating the ATE of Irrigation Event Executed on Field Soil Erosion Rate by covariate adjustment, which observed variables must \emph{not} be conditioned on? Return the forbidden set \texttt{\{"forbidden":[\dots]\}}, or \texttt{"no\_backdoor"} if no valid adjustment set exists but the ATE is otherwise identifiable, or \texttt{"non\_id"} if the ATE is not identifiable.%
}

\newcommand{\SceneVariableKey}{%
$Z$=irrigation subsidy (instr.), $X$=irrigation exec.\ (treat.), $Y$=soil erosion, $U$=soil permeability (latent).%
}

% The DAG is native TikZ. Edit nodes and edges here when substituting a scene.
\newcommand{\SceneDAG}{%
  \begin{tikzpicture}[
    x=1cm,y=1cm,
    every node/.style={font=\fontsize{8.5}{10}\selectfont},
    observed/.style={circle,draw=SceneGraphInk,fill=white,line width=.55pt,
      minimum size=5.8mm,inner sep=0pt},
    latent/.style={observed,dashed},
    causal/.style={-{Stealth[length=1.5mm,width=1.1mm]},
      draw=SceneGraphInk,line width=.55pt}]
    \node[observed] (Z) at (0,0) {$Z$};
    \node[observed] (X) at (1.1,0) {$X$};
    \node[observed] (Y) at (2.2,0) {$Y$};
    \node[latent] (U) at (1.65,.88) {$U$};
    \draw[causal] (Z) -- (X);
    \draw[causal] (X) -- (Y);
    \draw[causal] (U) -- (X);
    \draw[causal] (U) -- (Y);
  \end{tikzpicture}%
}


==> figs/scene_example_style.tex <==
% Helvetica at the selected mockup's scale, scoped to this figure's family.
% The manuscript's other sans-serif text keeps its existing font settings.
\DeclareFontFamily{T1}{SceneSans}{}
\DeclareFontShape{T1}{SceneSans}{m}{n}{<-> s*[.96] phvr8t}{}
\DeclareFontShape{T1}{SceneSans}{m}{it}{<-> s*[.96] phvro8t}{}
\DeclareFontShape{T1}{SceneSans}{b}{n}{<-> s*[.96] phvb8t}{}
\DeclareFontShape{T1}{SceneSans}{b}{it}{<-> s*[.96] phvbo8t}{}
\DeclareFontShape{T1}{SceneSans}{bx}{n}{<-> ssub * SceneSans/b/n}{}
\DeclareFontShape{T1}{SceneSans}{bx}{it}{<-> ssub * SceneSans/b/it}{}
\DeclareFontFamily{TS1}{SceneSans}{}
\DeclareFontShape{TS1}{SceneSans}{m}{n}{<-> s*[.96] phvr8c}{}
\DeclareFontShape{TS1}{SceneSans}{m}{it}{<-> s*[.96] phvro8c}{}
\DeclareFontShape{TS1}{SceneSans}{b}{n}{<-> s*[.96] phvb8c}{}
\DeclareFontShape{TS1}{SceneSans}{b}{it}{<-> s*[.96] phvbo8c}{}
\DeclareFontShape{TS1}{SceneSans}{bx}{n}{<-> ssub * SceneSans/b/n}{}
\DeclareFontShape{TS1}{SceneSans}{bx}{it}{<-> ssub * SceneSans/b/it}{}
\DeclareEncodingSubset{TS1}{SceneSans}{5}

% Native LaTeX/TikZ styling; font choices are inherited from the document.
% Requires: xcolor, tikz (arrows.meta), booktabs, array, colortbl, microtype.
\definecolor{SceneAccent}{HTML}{6B5ECF}
\definecolor{SceneInk}{HTML}{333239}
\definecolor{SceneMuted}{HTML}{69666D}
\definecolor{SceneRule}{HTML}{DAD7E0}
\definecolor{SceneWash}{HTML}{F8F8FA}
\definecolor{SceneGraphInk}{HTML}{62606B}

\newcommand{\SceneBodyFont}{\sffamily\fontsize{7.5}{8.8}\selectfont}
\newcommand{\SceneSmallFont}{\sffamily\fontsize{7}{8.4}\selectfont}
\newcommand{\SceneTableFont}{\sffamily\fontsize{7.1}{8.5}\selectfont}
\newcommand{\SceneBase}{%
  \color{SceneInk}\SceneBodyFont
  \setlength{\parindent}{0pt}\setlength{\parskip}{0pt}%
  \setlength{\emergencystretch}{1em}%
}
\newcommand{\SceneLabel}[1]{%
  {\sffamily\bfseries\fontsize{7.5}{8.8}\selectfont #1\par}\vspace{2pt}%
}
\newcommand{\SceneInlineLabel}[1]{{\bfseries #1.}\enspace}
\newcommand{\SceneSmallLabel}[1]{%
  {\sffamily\bfseries\fontsize{7.1}{8.5}\selectfont\color{SceneMuted}#1\par}\vspace{1pt}%
}
\newcommand{\SceneRuleLine}{\par\vspace{2pt}{\color{SceneRule}\hrule height .45pt}\vspace{2pt}}
\newcommand{\SceneHeader}{%
  {\sffamily\bfseries\fontsize{10}{11.8}\selectfont\SceneTitle\hfill
    {\normalfont\sffamily\fontsize{7.2}{9}\selectfont\color{SceneMuted}Scene example}\par}%
  \vspace{1pt}%
  {\sffamily\fontsize{6.9}{8.5}\selectfont\color{SceneMuted}\SceneMetadata\par}%
  \vspace{2pt}{\color{SceneAccent!65!black}\hrule height .7pt}\vspace{3pt}%
}
% colortbl sets rule color globally; restore it after this figure's table.
\makeatletter
\newcommand{\SceneDataTable}{%
  \begingroup\let\SceneSavedRuleColor\CT@arc@
  \SceneTableFont\setlength{\tabcolsep}{2.2pt}%
  \renewcommand{\arraystretch}{1}\arrayrulecolor{SceneRule}%
  \setlength{\aboverulesep}{1.5pt}\setlength{\belowrulesep}{1.5pt}%
  \begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}r rrr rrr@{}}
    \toprule[.5pt]
    Y & Z\_1 & Z\_2 & Z\_3 & X\_1 & X\_2 & X\_3 \\
    \cmidrule(lr){1-1}\cmidrule(lr){2-4}\cmidrule(lr){5-7}
    \SceneDataRows
    \bottomrule[.5pt]
  \end{tabular*}%
  \global\let\CT@arc@\SceneSavedRuleColor
  \endgroup
}
\makeatother
\newcommand{\ScenePrivatePanel}{%
  \SceneSmallLabel{Private ground-truth DAG}%
  {\centering\scalebox{.9}{\SceneDAG}\par}\vspace{1pt}%
  {\SceneSmallFont\raggedright\SceneVariableKey\par}%
}
\newcommand{\SceneTaskBand}{%
  \begingroup\setlength{\fboxsep}{3pt}%
  \colorbox{SceneWash}{%
    \begin{minipage}{\dimexpr\linewidth-2\fboxsep\relax}
      \SceneBase\SceneInlineLabel{Question}\SceneQuestion
    \end{minipage}}\par
  \endgroup
}

